Multi-Camera Visual-Inertial Simultaneous Localization and Mapping for Autonomous Valet Parking

Localization and mapping are key capabilities for self-driving vehicles. In this paper, we build on Kimera and extend it to use multiple cameras as well as external (eg wheel) odometry sensors, to obtain accurate and robust odometry estimates in real-world problems. Additionally, we propose an effective scheme for closing loops that circumvents the drawbacks of common alternatives based on the Perspective-n-Point method and also works with a single monocular camera. Finally, we develop a method for dense 3D mapping of the free space that combines a segmentation network for free-space detection with a homography-based dense mapping technique. We test our system on photo-realistic simulations and on several real datasets collected on a car prototype developed by the Ford Motor Company, spanning both indoor and outdoor parking scenarios. Our multi-camera system is shown to outperform state-of-the art open-source visual-inertial-SLAM pipelines (Vins-Fusion, ORB-SLAM3), and exhibits an average trajectory error under 1% of the trajectory length across more than 8km of distance traveled (combined across all datasets). A video showcasing the system is available at: youtu.be/H8CpzDpXOI8.

==> figures/extra/competitor_results.tex <==
\begin{table*}[h]
  \centering
  \caption{Accuracy of the State Estimation (vinsfusion vio)}
  \label{tab:accuracy_comparison}
  \begin{tabularx}{\textwidth}{l *{8}{Y}}
    \toprule
    & \multicolumn{8}{c}{APE Translation} \\
    \cmidrule{2-9}
    & \multicolumn{2}{c}{\textbf{VinsFusionFrontCam}} & \multicolumn{2}{c}{\textbf{VinsFusionLeftCam}} & \multicolumn{2}{c}{\textbf{VinsFusionRearCam}} & \multicolumn{2}{c}{\textbf{VinsFusionRightCam}}  \\
Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
 \midrule 
sim1 (187m)        & 2.7               & 1.5                 & \textbf{0.5}      & \textbf{0.3} & 2891.6           & 1269.5           & 1.1               & 0.5 \\
sim2 (351m)        & 1.6               & 0.5                 & 2.5               & 0.7          & 5044.6           & 1156.6           & \textbf{0.9}      & \textbf{0.2} \\
sim3 (618m)        & 8.1               & 1.3                 & 5.8               & 0.9          & 21359.8          & 2982.0           & \textbf{4.1}      & \textbf{0.6} \\
sim4 (612m)        & 6.3               & 1.0                 & 7.6               & 1.1          & 23790.9          & 3361.8           & \textbf{5.5}      & \textbf{0.7} \\
out0 (484m)        & 3721.3            & 768.1               & \textbf{25.5}     & \textbf{5.6} & 719.8            & 160.9            & 28.1              & 6.0 \\
out1 (332m)        & 20.3              & 6.1                 & 13370.2           & 3308.4       & 202.9            & 55.9             & \textbf{18.4}     & \textbf{4.7} \\
out2 (394m)        & 1268.8            & 321.6               & 12675.4           & 2508.2       & 1259.8           & 255.8            & \textbf{82.2}     & \textbf{16.9} \\
out3 (600m)        & 20.4              & 3.4                 & \textbf{12.2}     & \textbf{1.6} & 5652.0           & 760.7            & 16.1              & 2.2 \\
out4 (452m)        & \textbf{13.1}     & \textbf{2.9}        & 11117.1           & 2167.6       & 5393.6           & 1138.5           & 21.6              & 4.6 \\
out5 (277m)        & 5900.5            & 2127.5              & 47.1              & 11.8         & 12.1             & 3.2              & \textbf{9.8}      & \textbf{2.6} \\
in0 (339m)         & 8.2               & 2.4                 & 6.7               & 2.0          & 10.2             & 3.5              & \textbf{5.3}      & \textbf{1.5} \\
out6 (213m)        & 6.6               & 3.1                 & 10.3              & 2.8          & \textbf{3.3}     & \textbf{0.9}     & 38.2              & 10.2 \\
out7 (238m)        & \textbf{3.5}      & 1.5                 & 11.3              & 4.0          & 3.6              & \textbf{1.3}     & 5.1               & 1.6 \\
out8 (251m)        & \textbf{7.0}      & \textbf{2.8}        & 10.7              & 4.2          & 10.2             & 4.0              & 20.3              & 6.7 \\
out9 (199m)        & \textbf{2.6}      & \textbf{1.3}        & 7.1               & 3.6          & 5.3              & 1.8              & 13.9              & 4.7 \\
out10 (257m)       & 17.2              & 6.7                 & \textbf{9.6}      & 3.4          & 10.7             & \textbf{2.9}     & 17.2              & 4.8 \\
out11 (157m)       & \textbf{3.7}      & 2.3                 & 10.8              & 6.9          & 4.7              & \textbf{1.8}     & 15.3              & 6.2 \\
out12 (248m)       & 8.5               & 3.4                 & \textbf{5.7}      & \textbf{1.7} & 8.0              & 2.2              & 10.3              & 2.8 \\
out13 (165m)       & 1440.1            & 870.9               & 10.4              & 5.2          & \textbf{2.7}     & \textbf{1.2}     & 14.4              & 6.5 \\
in1 (273m)         & 5.8               & 2.1                 & 3.1               & 1.4          & \textbf{2.6}     & \textbf{1.1}     & 5.9               & 2.0 \\
out14 (284m)       & 8.6               & 3.0                 & 8.3               & 2.2          & \textbf{4.7}     & \textbf{1.3}     & 10.2              & 2.7 \\
out15 (108m)       & 2.9               & 2.6                 & 4.7               & 4.0          & \textbf{1.9}     & \textbf{1.5}     & 3.4               & 2.7 \\
in2 (483m)         & 13.7              & 2.8                 & 15.8              & 3.2          & \textbf{10.7}    & \textbf{2.4}     & 38.2              & 7.4 \\
in3 (136170484m)   & 113258534933581.9 & 83174070.8          & 622929647847936.1 & 344921422.4  & \textbf{28987.1} & \textbf{14657.2} & 416605236335120.6 & 264027001.4 \\
in4 (712m)         & 872.4             & 122.5               & 22.4              & 3.1          & \textbf{15.6}    & \textbf{2.3}     & 18.5              & 2.6 \\
in5 (638m)         & 34.1              & 5.3                 & 18.4              & 2.9          & \textbf{13.2}    & \textbf{2.1}     & 30.2              & 4.8 \\

    \bottomrule
  \end{tabularx}%
\end{table*}{}


\begin{table*}[h]
  \centering
  \caption{Accuracy of the State Estimation (vinsfusion pgo)}
  \label{tab:accuracy_comparison}
  \begin{tabularx}{\textwidth}{l *{8}{Y}}
    \toprule
    & \multicolumn{8}{c}{APE Translation} \\
    \cmidrule{2-9}
    & \multicolumn{2}{c}{\textbf{VinsFusionFrontCam}} & \multicolumn{2}{c}{\textbf{VinsFusionLeftCam}} & \multicolumn{2}{c}{\textbf{VinsFusionRearCam}} & \multicolumn{2}{c}{\textbf{VinsFusionRightCam}}  \\
Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
 \midrule 
sim1 (241m)        & 2.7               & 1.1           & \textbf{0.6}      & \textbf{0.2}  & 3461.8                     & 1459.0              & 1.1                 & 0.4           \\
sim2 (460m)        & 1.7               & 0.4           & 2.4               & 0.5           & 5511.5                     & 1205.7              & \textbf{1.1}        & \textbf{0.2}  \\
sim3 (737m)        & 7.0               & 1.0           & 5.7               & 0.8           & 24801.8                    & 3390.9              & \textbf{4.0}        & \textbf{0.5}  \\
sim4 (800m)        & 8.1               & 1.0           & 8.6               & 1.1           & 29418.8                    & 3806.3              & \textbf{6.6}        & \textbf{0.8}  \\ 
out0 (496m)        & 4347.5            & 876.3         & \textbf{28.1}     & \textbf{5.7}  & 863.5                      & 174.1               & 29.4                & 5.9           \\
out1 (443m)        & 18.3              & 4.1           & 15418.2           & 3466.4        & 229.9                      & 51.7                & \textbf{16.3}       & \textbf{3.7}  \\
out2 (516m)        & 1697.0            & 328.5         & 14039.3           & 2702.0        & 1411.0                     & 272.3               & \textbf{80.8}       & \textbf{15.6} \\
out3 (805m)        & 20.9              & 2.6           & \textbf{11.5}     & \textbf{1.4}  & 6786.7                     & 842.9               & 14.5                & 1.8           \\
out4 (534m)        & \textbf{15.7}     & \textbf{2.9}  & 12860.4           & 2403.6        & 7168.2                     & 1339.9              & 22.5                & 4.2           \\
out5 (513m)        & 8082.3            & 1574.5        & 88.0              & 17.2          & 15.1                       & 3.0                 & \textbf{9.8}        & \textbf{1.9}  \\
out6 (448m)        & 6.2               & 1.4           & 9.8               & 2.2           & \textbf{3.4}               & \textbf{0.8}        & 42.1                & 9.6           \\
out7 (405m)        & \textbf{3.7}      & \textbf{0.9}  & 9.9               & 2.4           & 4.1                        & 1.0                 & 5.2                 & 1.3           \\
out8 (355m)        & \textbf{6.5}      & \textbf{1.8}  & 10.6              & 3.0           & 12.2                       & 3.4                 & 20.1                & 5.6           \\
out9 (414m)        & \textbf{2.4}      & \textbf{0.6}  & 7.7               & 1.9           & 5.2                        & 1.3                 & 13.9                & 3.3           \\
out10 (486m)       & 19.5              & 4.0           & \textbf{8.4}      & \textbf{1.7}  & 14.3                       & 2.9                 & 17.9                & 3.7           \\
out11 (414m)       & \textbf{4.3}      & \textbf{1.0}  & 11.3              & 2.7           & 7.9                        & 1.9                 & 14.1                & 3.4           \\
out12 (437m)       & 7.6               & 1.7           & \textbf{6.7}      & \textbf{1.5}  & 7.5                        & 1.7                 & 9.8                 & 2.2           \\
out13 (341m)       & 1643.9            & 481.6         & 10.4              & 3.0           & \textbf{3.3}               & \textbf{1.0}        & 18.8                & 5.5           \\
out14 (517m)       & 9.6               & 1.9           & 8.1               & 1.6           & \textbf{5.3}               & \textbf{1.0}        & 10.0                & 1.9           \\
out15 (194m)       & 3.4               & 1.8           & 4.1               & 2.1           & \textbf{2.0}               & \textbf{1.0}        & 3.8                 & 2.0           \\
in0 (420m)         & 10.2              & 2.4           & 7.5               & 1.8           & 10.4                       & 2.5                 & \textbf{5.4}        & \textbf{1.3}  \\
in1 (321m)         & 6.6               & 2.1           & 3.4               & 1.1           & \textbf{2.7}               & \textbf{0.8}        & 5.8                 & 1.8           \\
in2 (562m)         & 17.5              & 3.1           & 19.3              & 3.4           & \textbf{13.2}              & \textbf{2.3}        & 41.5                & 7.4           \\
in3 (232999894m)   & 203636501100747.9 & 87397679.6    & 767959170790861.0 & 330144570.2   & \textbf{110890570796298.5} & \textbf{47671700.7} & 552910741745630.6 & 237300854.9     \\
in4 (723m)         & 918.6             & 126.9         & 23.0              & 3.2           & \textbf{16.3}              & \textbf{2.3}        & 18.6                & 2.6           \\
in5 (647m)         & 35.4              & 5.5           & 17.9              & 2.8           & \textbf{15.3}              & \textbf{2.4}        & 31.7                & 4.9           \\

    \bottomrule
  \end{tabularx}%
\end{table*}{}


\begin{table*}[h]
  \centering
  \caption{Accuracy of the State Estimation (openvins)}
  \label{tab:accuracy_comparison}
  \begin{tabularx}{\textwidth}{l *{8}{Y}}
    \toprule
    & \multicolumn{8}{c}{APE Translation} \\
    \cmidrule{2-9}
    & \multicolumn{2}{c}{\textbf{FrontCam}} & \multicolumn{2}{c}{\textbf{LeftCam}} & \multicolumn{2}{c}{\textbf{RearCam}} & \multicolumn{2}{c}{\textbf{RightCam}}  \\
Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
 \midrule 
sim1 (249m)       & \textbf{12.9}  & \textbf{5.2}  & 15.0            & 6.0             & 92.1           & 36.9          & 17.5          & 7.0 \\
sim2 (466m)       & 21103.9        & 4525.7        & \textbf{9187.1} & \textbf{1970.3} & 24136.3        & 5176.0        & 13116.2       & 2812.8 \\
sim3 (749m)       & 23.0           & 3.1           & \textbf{5.0}    & \textbf{0.7}    & 12.5           & 1.7           & 7.3           & 1.0 \\
sim4 (804m)       & 26.0           & 3.2           & 17.0            & 2.1             & \textbf{11.5}  & \textbf{1.4}  & 19.9          & 2.5 \\ 
out0 (496m)       & 232.1          & 46.8          & \textbf{112.2}  & \textbf{22.6}   & 3174.2         & 640.0         & 511.7         & 103.2 \\
out1 (444m)       & 4523.9         & 1017.4        & 419.7           & 94.4            & \textbf{82.0}  & \textbf{18.4} & 5536.6        & 1245.1 \\
out2 (519m)       & \textbf{32.8}  & \textbf{6.3}  & 42.1            & 8.1             & 17394.7        & 3350.5        & 35.8          & 6.9 \\
out3 (805m)       & 840.7          & 104.3         & 16299.9         & 2023.2          & \textbf{55.4}  & \textbf{6.9}  & 1993.9        & 247.5 \\
out4 (534m)       & \textbf{151.7} & \textbf{28.4} & 13811.7         & 2581.7          & 1640.4         & 306.6         & 1298.2        & 242.7 \\
out5 (513m)       & 3280.3         & 639.1         & \textbf{96.5}   & \textbf{18.8}   & 265.4          & 51.7          & 2361.5        & 460.0 \\
in0 (422m)        & 57.6           & 13.7          & 81.6            & 19.3            & \textbf{18.0}  & \textbf{4.3}  & 52.1          & 12.3 \\
out6 (448m)       & 49.1           & 10.9          & \textbf{17.0}   & \textbf{3.8}    & 41.2           & 9.2           & 31.4          & 7.0 \\
out7 (406m)       & 156.4          & 38.5          & \textbf{22.2}   & \textbf{5.5}    & 40.7           & 10.0          & 67.0          & 16.5 \\
out8 (356m)       & 69.6           & 19.5          & \textbf{18.1}   & \textbf{5.1}    & 74.0           & 20.7          & 143.4         & 40.2 \\
out9 (415m)       & 56.4           & 13.6          & \textbf{13.3}   & \textbf{3.2}    & 94.8           & 22.8          & 169.6         & 40.8 \\
out10 (486m)      & 108.6          & 22.3          & 35.0            & 7.2             & \textbf{34.6}  & \textbf{7.1}  & 156.3         & 32.1 \\
out11 (415m)      & 67.7           & 16.3          & \textbf{20.3}   & \textbf{4.9}    & 48.4           & 11.6          & 201.0         & 48.4 \\
out12 (437m)      & 91.2           & 20.8          & 45.1            & 10.3            & 30.5           & 7.0           & \textbf{21.1} & \textbf{4.8} \\
out13 (341m)      & 12.6           & 3.7           & 15.1            & 4.4             & \textbf{9.8}   & \textbf{2.9}  & 27.3          & 8.0 \\
in1 (321m)        & 28.7           & 8.9           & 79.8            & 24.8            & \textbf{26.1}  & \textbf{8.1}  & 147.3         & 45.8 \\
out14 (518m)      & 190.5          & 36.8          & \textbf{33.5}   & \textbf{6.5}    & 144.2          & 27.8          & 197.2         & 38.0 \\
out15 (194m)      & 15.9           & 8.2           & \textbf{7.2}    & \textbf{3.7}    & 32.0           & 16.4          & 15.1          & 7.8 \\
in2 (565m)        & \textbf{58.4}  & \textbf{10.3} & 97.2            & 17.2            & 85.3           & 15.1          & 65.6          & 11.6 \\
in3 (416m)        & 46.5           & 11.2          & 63.1            & 15.1            & \textbf{24.4}  & \textbf{5.9}  & 59.3          & 14.2 \\
in4 (724m)        & \textbf{56.1}  & \textbf{7.7}  & 191.1           & 26.4            & 120.4          & 16.6          & 147.2         & 20.3 \\
in5 (647m)        & 207.2          & 32.0          & 420.5           & 64.9            & 61.6           & 9.5           & \textbf{37.5} & \textbf{5.8} \\

    \bottomrule
  \end{tabularx}%
\end{table*}{}


\begin{table*}[h]
  \centering
  \caption{Accuracy of the State Estimation (orbslam3)}
  \label{tab:accuracy_comparison}
  \begin{tabularx}{\textwidth}{l *{8}{Y}}
    \toprule
    & \multicolumn{8}{c}{APE Translation} \\
    \cmidrule{2-9}
    & \multicolumn{2}{c}{\textbf{FrontCam}} & \multicolumn{2}{c}{\textbf{LeftCam}} & \multicolumn{2}{c}{\textbf{RearCam}} & \multicolumn{2}{c}{\textbf{RightCam}}  \\
Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
 \midrule 
sim1 (250m)       & 39.3  & 15.7         & 37.0           & 14.8          & 35.1          & 14.0          & \textbf{33.6} & \textbf{13.4} \\
sim2 (468m)       & 39.2  & 8.4          & 35.8           & 7.6           & \textbf{22.6} & \textbf{4.8}  & 40.7          & 8.7 \\
sim3 (749m)       & 70.1  & 9.4          & 71.4           & 9.5           & \textbf{61.2} & \textbf{8.2}  & 68.2          & 9.1 \\
sim4 (804m)       & 78.2  & 9.7          & 78.6           & 9.8           & \textbf{15.3} & \textbf{1.9}  & 79.5          & 9.9 \\
out0 (498m)       & 172.9 & 34.7         & \textbf{147.5} & \textbf{29.6} & 169.3         & 34.0          & 171.6         & 34.4 \\
out1 (445m)       & 44.4  & 10.0         & 43.6           & 9.8           & \textbf{43.1} & \textbf{9.7}  & 44.3          & 9.9 \\
out2 (521m)       & 46.8  & 9.0          & 43.8           & 8.4           & 46.9          & 9.0           & \textbf{43.2} & \textbf{8.3} \\
out3 (807m)       & 60.4  & 7.5          & \textbf{17.6}  & \textbf{2.2}  & 59.3          & 7.3           & 59.0          & 7.3 \\
out4 (536m)       & 165.2 & 30.8         & \textbf{19.2}  & \textbf{3.6}  & 167.3         & 31.2          & 26.2          & 4.9 \\
out5 (514m)       & 142.9 & 27.8         & 15.5           & 3.0           & \textbf{2.9}  & \textbf{0.6}  & 24.8          & 4.8 \\
in0 (421m)        & 22.6  & 5.4          & 3.6            & 0.8           & \textbf{2.8}  & \textbf{0.7}  & 14.0          & 3.3 \\
out6 (448m)       & 38.5  & 8.6          & \textbf{37.8}  & \textbf{8.4}  & 39.0          & 8.7           & 39.5          & 8.8 \\
out7 (406m)       & 34.5  & 8.5          & \textbf{8.9}   & \textbf{2.2}  & 12.5          & 3.1           & 11.5          & 2.8 \\
out8 (356m)       & 22.3  & 6.2          & 12.7           & 3.6           & 21.7          & 6.1           & \textbf{11.2} & \textbf{3.1} \\
out9 (415m)       & 10.6  & 2.5          & \textbf{6.4}   & \textbf{1.5}  & 9.1           & 2.2           & 9.6           & 2.3 \\
out10 (486m)      & 36.2  & 7.4          & 10.5           & 2.2           & \textbf{5.3}  & \textbf{1.1}  & 24.1          & 4.9 \\
out11 (415m)      & 19.8  & 4.8          & \textbf{9.0}   & \textbf{2.2}  & 32.4          & 7.8           & 90.9          & 21.9 \\
out12 (52m)       & 36.1  & 8.3          & \textbf{0.9}   & \textbf{1.8}  & 1.2           & 2.4           & 1.1           & 2.2 \\
out13 (341m)      & 20.3  & 5.9          & \textbf{11.9}  & \textbf{3.5}  & 20.1          & 5.9           & 23.8          & 7.0 \\
in1 (321m)        & 15.2  & 4.7          & \textbf{7.2}   & \textbf{2.2}  & 23.5          & 7.3           & 16.9          & 5.2 \\
out14 (518m)      & 48.2  & 9.3          & \textbf{20.9}  & \textbf{4.0}  & 48.7          & 9.4           & 45.5          & 8.8 \\
out15 (195m)      & 24.5  & 12.6         & 4.7            & 2.4           & \textbf{1.7}  & \textbf{0.9}  & 80.5          & 41.3 \\
in2 (565m)        & 49.7  & \textbf{8.8} & 43.4           & 15.4          & \textbf{41.2} & 14.7          & 53.9          & 9.5 \\
in3 (417m)        & 46.5  & 11.0         & 48.1           & 11.5          & 27.0          & 6.5           & \textbf{19.3} & \textbf{4.6} \\
in4 (725m)        & 51.2  & 7.1          & 50.6           & 7.0           & \textbf{39.7} & \textbf{5.5}  & 73.0          & 10.1 \\
in5 (648m)        & 43.7  & 6.7          & \textbf{33.0}  & \textbf{5.1}  & 53.1          & 8.2           & 53.0          & 8.2 \\

    \bottomrule
  \end{tabularx}%
\end{table*}{}


==> figures/extra/wheel_odom.tex <==
%!TEX root = ../../main.tex

% imu0noisy
% \begin{table}[h]
%     \centering
%     \caption{Accuracy of the State Estimation - VIO vs Wheel Odometry}
%     \label{tab:wheel_odom_comparison}
%     \begin{tabularx}{\columnwidth}{l *{6}{Y}}
%       \toprule
%       & \multicolumn{6}{c}{APE Translation} \\
%       \cmidrule{2-7}
%       & \multicolumn{2}{c}{\textbf{1cam}} & \multicolumn{2}{c}{\textbf{1cam + Wheel}} & \multicolumn{2}{c}{\textbf{Wheel Odometry}}  \\
%   Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
%    \midrule 
%     out0 (498 m) & 6.1 & 1.2 & \textcolor{green}{1.8} & \textcolor{green}{0.4} & 2.7 & 0.5 \\
%     out1 (445 m) & 3.5 & 0.8 & \textcolor{green}{0.7} & \textcolor{green}{0.2} & 2.5 & 0.6 \\
%     out2 (521 m) & 3.3 & 0.6 & \textcolor{green}{0.7} & \textcolor{green}{0.1} & 2.2 & 0.4 \\
%     out3 (807 m) & 6.7 & 0.8 & \textcolor{green}{1.1} & \textcolor{green}{0.1} & 3.0 & 0.4 \\
%     out4 (537 m) & \textcolor{green}{1.3} & \textcolor{green}{0.2} & 1.5 & 0.3 & 2.7 & 0.5 \\
%     out5 (514 m) & 26.7 & 5.2 & \textcolor{green}{1.7} & \textcolor{green}{0.3} & 2.0 & 0.4 \\
%     out6 (406 m) & 3.6 & 0.9 & \textcolor{green}{1.2} & \textcolor{green}{0.3} & 1.4 & 0.3 \\
%     out7 (48 m) & 0.3 & 0.6 & \textcolor{green}{0.3} & \textcolor{green}{0.6} & 0.5 & 1.1 \\
%     out8 (415 m) & 2.0 & 0.5 & \textcolor{green}{1.2} & \textcolor{green}{0.3} & 1.3 & 0.3 \\
%     out9 (486 m) & 2.0 & 0.4 & \textcolor{green}{1.1} & \textcolor{green}{0.2} & 1.6 & 0.3 \\
%     out10 (44 m) & 0.7 & 1.5 & \textcolor{green}{0.3} & \textcolor{green}{0.7} & 0.7 & 1.5 \\
%     out11 (437 m) & 2.4 & 0.6 & \textcolor{green}{1.1} & \textcolor{green}{0.2} & 1.5 & 0.3 \\
%     out12 (448 m) & 2.6 & 0.6 & \textcolor{green}{1.0} & \textcolor{green}{0.2} & 2.2 & 0.5 \\
%     out13 (341 m) & 1.5 & 0.4 & \textcolor{green}{0.9} & \textcolor{green}{0.3} & 1.3 & 0.4 \\
%     out14 (517 m) & 1.4 & 0.3 & \textcolor{green}{0.9} & \textcolor{green}{0.2} & 1.4 & 0.3 \\
%     out15 (194 m) & 1.1 & 0.6 & \textcolor{green}{0.2} & \textcolor{green}{0.1} & 1.1 & 0.5 \\
%    \bottomrule
% \end{tabularx}%
% \end{table}{}


% imu0
\begin{table}[h]
  \centering
  \caption{Accuracy of the State Estimation - VIO vs Wheel Odometry}
  \label{tab:wheel_odom_comparison}
  \begin{tabularx}{\columnwidth}{l *{6}{Y}}
    \toprule
    & \multicolumn{6}{c}{APE Translation} \\
    \cmidrule{2-7}
    & \multicolumn{2}{c}{\textbf{1cam}} & \multicolumn{2}{c}{\textbf{1cam + Wheel}} & \multicolumn{2}{c}{\textbf{Wheel Odometry}}  \\
    Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
 \midrule 
  out0 (498 m) & 4.2 & 0.8 & \textcolor{green}{1.8} & \textcolor{green}{0.4} & 2.7 & 0.5 \\
  out1 (445 m) & 4.6 & 1.0 & \textcolor{green}{0.7} & \textcolor{green}{0.2} & 2.5 & 0.6 \\
  out2 (521 m) & 3.6 & 0.7 & \textcolor{green}{0.6} & \textcolor{green}{0.1} & 2.2 & 0.4 \\
  out3 (807 m) & 4.7 & 0.6 & \textcolor{green}{1.0} & \textcolor{green}{0.1} & 3.0 & 0.4 \\
  out4 (537 m) & 1.6 & 0.3 & \textcolor{green}{1.5} & \textcolor{green}{0.3} & 2.7 & 0.5 \\
  out5 (514 m) & 5.5 & 1.1 & \textcolor{green}{1.9} & \textcolor{green}{0.4} & 2.0 & 0.4 \\
  out6 (406 m) & 3.3 & 0.8 & \textcolor{green}{1.3} & \textcolor{green}{0.3} & 1.4 & 0.3 \\
  out7 (356 m) & 1.9 & 0.5 & 1.6 & 0.4 & \textcolor{green}{1.2} & \textcolor{green}{0.3} \\
  out8 (415 m) & 3.5 & 0.8 & \textcolor{green}{1.3} & \textcolor{green}{0.3} & 1.3 & 0.3 \\
  out9 (486 m) & 1.8 & 0.4 & \textcolor{green}{1.2} & \textcolor{green}{0.2} & 1.6 & 0.3 \\
  out10 (415 m) & 3.4 & 0.8 & \textcolor{green}{1.2} & \textcolor{green}{0.3} & 1.4 & 0.3 \\
  out11 (437 m) & 1.6 & 0.4 & \textcolor{green}{1.0} & \textcolor{green}{0.2} & 1.5 & 0.3 \\
  out12 (448 m) & 3.3 & 0.7 & \textcolor{green}{1.0} & \textcolor{green}{0.2} & 2.2 & 0.5 \\
  out13 (341 m) & 0.9 & 0.3 & \textcolor{green}{0.9} & \textcolor{green}{0.3} & 1.3 & 0.4 \\
  out14 (517 m) & 1.4 & 0.3 & \textcolor{green}{0.8} & \textcolor{green}{0.2} & 1.4 & 0.3 \\
  out15 (194 m) & 1.3 & 0.7 & \textcolor{green}{0.3} & \textcolor{green}{0.2} & 1.1 & 0.5 \\
    \bottomrule
  \end{tabularx}%
\end{table}{}

==> figures/figure_car.tex <==
%!TEX root = ../main.tex

\begin{figure}[h]
% \vspace{-10mm}
    \includegraphics[width=\columnwidth]{img/car-setup.png}%
    \caption{An illustration of the Ford test bed and sensor setup.}
    \label{fig:car}
\vspace{-8mm}
\end{figure}


==> figures/table_robust_ablation.tex <==
%!TEX root = ../../main.tex

\begin{table}[h!]
  \centering
  \scriptsize
  \begin{tabularx}{\columnwidth}{l *{4}{Y}}
  \toprule
  & \multicolumn{4}{c}{\specialcell[b]{Robust Triangulation Factor Ablation Study \\ APE Translation}} \\
  \cmidrule{2-5}
  & \multicolumn{2}{c}{\textbf{Robust Noise Factor}} & \multicolumn{2}{c}{\textbf{Normal Noise Factor}}  \\
  Dataset &RMSE [m] & Drift [\%] & RMSE [m] & Drift [\%]  \\
  \midrule
  sim0 (250m)  & 1.1                     & 0.4                    & \textcolor{green}{1.0} & \textcolor{green}{0.4}  \\
  sim1 (467m)  & 0.9                     & 0.2                    & \textcolor{green}{0.7} & \textcolor{green}{0.1}  \\
  sim2 (749m)  & \textcolor{green}{2.2}  & \textcolor{green}{0.3} & 3.0                    & 0.4                     \\
  sim3 (804m)  & 1004.1                  & 124.9                  & \textcolor{green}{2.0} & \textcolor{green}{0.3}  \\
  \midrule
  out0 (498m)  & 6.1                     & 1.2                    & \textcolor{green}{0.7} & \textcolor{green}{0.1}  \\
  out1 (445m)  & \textcolor{green}{4.0}  & \textcolor{green}{0.9} & 4.4                    & 1.0                     \\
  out2 (521m)  & 3.3                     & 0.6                    & \textcolor{green}{2.8} & \textcolor{green}{0.5}  \\
  out3 (807m)  & \textcolor{green}{7.2}  & \textcolor{green}{0.9} & 7.5                    & 0.9                     \\
  out4 (537m)  & 1.3                     & 0.2                    & \textcolor{green}{0.8} & \textcolor{green}{0.2}  \\
  out5 (514m)  & 29.4                    & 5.7                    & \textcolor{green}{20.5} & \textcolor{green}{4.0} \\
  out6 (448m)  & 3.0                     & 0.7                    & \textcolor{green}{2.9} & \textcolor{green}{0.6}  \\
  out7 (406m)  & 3.9                     & 1.0                    & \textcolor{green}{3.1} & \textcolor{green}{0.8}  \\
  out8 (48m)   & \textcolor{green}{0.3}  & \textcolor{green}{0.6} & 0.3                    & 0.7                     \\
  out9 (415m)  & \textcolor{green}{1.5}  & \textcolor{green}{0.4} & 2.2                    & 0.5                     \\
  out10 (486m) & \textcolor{green}{2.1}  & \textcolor{green}{0.4} & 2.3                    & 0.5                     \\
  out11 (44m)  & 0.7                     & 1.5                    & \textcolor{green}{0.5} & \textcolor{green}{1.2}  \\
  out12 (437m) & 2.5                     & 0.6                    & \textcolor{green}{2.1} & \textcolor{green}{0.5}  \\
  out13 (341m) & \textcolor{green}{1.3}  & \textcolor{green}{0.4} & 1.4                    & 0.4                     \\
  out14 (517m) & 1.7                     & 0.3                    & \textcolor{green}{1.3} & \textcolor{green}{0.2}  \\
  out15 (194m) & 1.1                     & 0.6                    & \textcolor{green}{1.0} & \textcolor{green}{0.5}  \\
  \midrule
  in0 (421m)   & 3.0                     & 0.7                    & \textcolor{green}{2.8} & \textcolor{green}{0.7}  \\
  in1 (321m)   & \textcolor{green}{4.3}  & \textcolor{green}{1.4} & 4.9                    & 1.5                     \\
  in2 (563m)   & \textcolor{green}{10.0} & \textcolor{green}{1.8} & 11.4                   & 2.0                     \\
  in3 (417m)   & \textcolor{green}{11.1} & \textcolor{green}{2.7} & 14.0                   & 3.4                     \\
  in4 (723m)   & 8.9                     & 1.2                    & \textcolor{green}{8.5} & \textcolor{green}{1.2}  \\
  in5 (647m)   & 11.4                    & 1.8                    & \textcolor{green}{9.9} & \textcolor{green}{1.5}  \\
  \bottomrule
\end{tabularx}%
\caption{Ablation study on Robust Smart Noise Factor using the right-camera monocular-VIO configuration.}
\label{tab:kimera_robust_ablation}
\end{table}{}


==> preamble_algo.tex <==
%!TEX root = main.tex
\lstdefinelanguage{mine} 
{morekeywords={while,True,if,break,=,return,function,for,until,in,input,output,assumptions,assumption,invariant,loop,variant,end,invariant,precondition,variables}, 
sensitive=false, 
morecomment=[l]{\#}, 
morecomment=[il]\%{.}, 
morecomment=[s]{/*}{*/}, 
morestring=[b]", 
} 

\lstset{% general command to set parameter(s) 
basicstyle=\small\rmfamily, % print whole listing small 
keywordstyle=\color{black}\bfseries, 
% underlined bold black keywords 
identifierstyle=, % nothing happens 
commentstyle=\color[rgb]{0.2,0.2,0.2},
stringstyle=\ttfamily, % typewriter type for strings 
showstringspaces=false,
mathescape=true,
fontadjust=true,
columns=fullflexible} % no special string spaces 
\lstset{frameround=fttt,frame=none}

\usepackage{calc}
\newlength\listingnumberwidth
\setlength\listingnumberwidth{\widthof{00}}
\lstset{
numbers=left,
xleftmargin=\listingnumberwidth,
numbersep=1em
}


\lstset{escapeinside={*@}{@*}}

\newcommand{\tuple}[2]{\langle#1,#2\rangle}
